When to Ask for Help: Proactive Interventions in Autonomous Reinforcement Learning

A long-term goal of reinforcement learning is to design agents that can autonomously interact and learn in the world. A critical challenge to such autonomy is the presence of irreversible states which require external assistance to recover from, such as when a robot arm has pushed an object off of a table. While standard agents require constant monitoring to decide when to intervene, we aim to design proactive agents that can request human intervention only when needed. To this end, we propose an algorithm that efficiently learns to detect and avoid states that are irreversible, and proactively asks for help in case the agent does enter them. On a suite of continuous control environments with unknown irreversible states, we find that our algorithm exhibits better sample- and intervention-efficiency compared to existing methods. Our code is publicly available at https://sites.google.com/view/proactive-interventions

==> comments.tex <==
%%CF.4.30: I think it would be nice to focus this paragraph on laying out the goal/vision of this work without talking about what prior works do. (though using references to support text where needed). You can leave the prior works to the next paragraph. This could go roughly as follows: 
% we want an agent to learn behavior through autonomously exploring in and interacting with its environment
% in many realistic settings, such an agent will inevitably reach a state from which it cannot recover, an irreversible state, during the learning process. (side note: does it make sense to use the term "irreversible" like that? it seems like irreversible is an adjective that should modify an action not a state... though it would be nice to have some terminology for these states...)
% give an example, ideally one in our experiments like a robot arm accidentally pushing an object off the table
% in such settings, the robot should proactively reach out for help, e.g. by taking a special course of action that contacts a human supervisor or another agent.
% in this paper, our goal is to develop algorithms that allow for this kind of behavior: that enable agents to detect irreversible states, proactively request an intervention, and otherwise learn autonomously.
%%CF.4.30: I think that this opening paragraph is more interesting and more vivid than the current paragraph. Then, after such an opening paragraph, the second paragraph could then focus on how prior methods do and do not address aspects of this problem -- mentioning how many ARL methods learn autonomously without resets but generally assume ergodic environments. and on the other hand, methods for safe RL develop approaches for avoiding particular parts of the state space but assume that the agent is told precisely when it reaches such parts of the state space.
% In the real world, an autonomous agent has to contend with the consequences of its own actions. 
%%CF.4.30: This first sentence doesn't seem that inspiring. :)
% AS.5.13: Try something like -- the world doesn't always offer second chances. How do we learn in presence of irreversibilities?...
% For example, an agent learning how to shelf a book will need to pick up the book if it drops it, unlike simulated environments where the agent can be reset to a state where the book is grasped. \annie{Maybe use one of our experimental tasks as the example} 
%%CF.4.30: +1 
% Such resetting of the environments can entail expensive human supervision and thus, several recent works have focused on efficiently learning behaviors with minimal access to resetting mechanisms~\citep{han2015learning, zhu2020ingredients, sharma2021autonomouscurr}. However, these prior works have implicitly assumed reversible environments where it is always feasible for an agent to revert any sequence of actions, an assumption that often doesn’t hold. For example, how can a robot arm continue improving its mug grasping policy if it has pushed the mug out of its reach? \annie{and keep the example consistent?}
%%CF.4.30: +1
%%CF.4.30: Also, Annie you should feel free to make revisions yourself too!

% For environments where an agent may encounter irreversible states, extrinsic interventions become necessary for the agent to continue optimizing the task performance. To minimize human supervision in the form of interventions required while training in such environments, it is desirable that the agent: (a) operates autonomously without requiring interventions as long as possible and (b) learns to avoid irreversible states. 
%%CF.4.30: It would be really nice if the above kind of content (i.e. info about the problem we're trying to solve) went in this first paragraph so that this paragraph can focus on how prior works don't solve this problem.
% A related desiderata arises in context of safe reinforcement learning (RL) ~\citep{garcia2015comprehensive},
%%CF.4.30: should generally have more than one cite for this class of methods in the intro
% where the objective is to maximize task performance while minimizing violations of safety constraints, as given by an indicator function $\mathcal{I}^{\textit{safe}}(s)$ that specifies whether a state is safe or not.
% \annie{I feel like if we are going to start using notation here, maybe we should just give a more formal definition of the indicator function, i.e., $\mathcal{I}^{\textit{safe}}(s) = \{ s \in \mathcal{S}^\textit{safe} \}$}
% AS: I am trying to emphasize that safety and reversibility are not the same problems.
% AS: We can switch the name if needed
%%CF.4.30: I think it would be nice to avoid notation in the intro like this. I don't think it's necessary to communicate clearly, and may make it less clear and more clunky because it will inevitably rely on notational preliminaries that we haven't covered yet.
% Given access to an analogous indicator of reversibility $\mathcal{I}^{\textit{rev}}(s)$, the agent can request an intervention whenever it is an irreversible state, that is $\mathcal{I}^{\textit{rev}}(s) = 0$ to satisfy desiderata (a), and leverage algorithmic techniques from safe RL to avoid irreversible states to satisfy desiderata (b). However, an oracle $\mathcal{I}^{\textit{rev}}(s)$ is rarely available and specifying such a function for large continuous state-spaces, possibly high-dimensional such as images, can be cumbersome.
%%CF.4.30: Right now, the text takes quite a few sentences to get to the point, and I think there's a clearer and more concise way to phrase it. e.g. "Methods for safe RL develop approaches for avoiding particular parts of the state space~\cite{stuff}. However, these methods assume that the agent is told precisely when it reaches such parts of the state space. In contrast, an autonomous agent may not know when it has reached an irreversible state (such as knocking an important object off a table), and an algorithm in this setting should instead learn to detect such states while minimizing queries about whether a state is reversible."
% Unfortunately, detecting when to call for a human intervention is a non-trivial problem itself. A similar problem arises in context of safe reinforcement learning where the agent learns how to solve the task in presence of constraints. However, such

% Instead of assuming oracle access to $\mathcal{I}^{\textit{rev}}(s)$, what if we query the function for labels online? 


%%CF.5.17: I don't think this sentence is particularly formal. Maybe "Concretely, "? not sure.
%%CF.5.17: also, when you spell out method names, they should be lowercase (only the acronym should be uppercase)
% for developing RL algorithms 
%%CF.4.30: we propose an RL framework for developing RL methods? awk phrasing
% for environments with potentially irreversible states,
% Second, we propose an algorithm
%%CF.4.30: how is the framework different from the algorithm? this could be more clear

%%CF.4.30: this seems redundant with previous paragraph.


% Third, we propose multiple rules to determine when an agent should request an extrinsic intervention to reset the environment based on our proposed framework.
%%CF.4.30: I don't think we need to list all of these as separate contributions. I think the writing would be stronger if we simply say that "our main contribution is a framework/method, <method name>, that enables agents to ..." Then, briefly mention any secondary contributions or benefits of this like any theory and/or applicability to multiple RL algorithms. Then, summarize the experimental results.
% And finally, we combine all the component to propose algorithm(s) XXX 
%%CF.4.30: weren't we already proposing an algorithm?
% for learning behaviors in a non-episodic environments with irreversible states. Our experiments and analysis demonstrate ...

%%CF.5.17: should revise phrasing here based on Ben's feedback. Maybe "queries to an oracle" -> "label queries" or "queries for a reversibility label"



% Related Work

%%CF.4.30: Does it make sense to compare to one of these methods? As stated, it seems like these methods are extremely relevant. 

%%CF.4.30: To avoid the attentive supervision needed for episodic resets, prior work..."

%%CF.4.30: "the MDP the agent learns in" -> the agent's environment

%%CF.4.30: make it explicitly clear that this is what we aim to do. e.g. "Most autonomous RL work assumes the agent's environment is ergodic and thus reversible, whereas we specifically aim to tackle the setting where this is not the case." 

% Deployment of RL algorithms on real systems often requires human-supervised resets~\citep{finn2016deep,gu2017deep,ghadirzadeh2017deep} or clever design of a reset mechanism~\citep{zhu2019dexterous,nagabandi2020deep,sharma2020emergent}. 
%%CF.4.30: not sure if you need this first sentence. though, I do think it is good to make it clear why standard RL methods aren't autonomous in practice. Maybe you could instead start this as "Multiple prior works have also studied autonomy in RL, motivated by the fact that deployments of RL algorithms on real robots often require human-provided resets at the end of each episode~\cite{stuff}." I think that would both be a smoother transition and get across how RL is not autonomous. I think you can skip the reset mechanism part because technically that does make it autonomous, and it's not that important.

%%CF.4.30: should add MEDAL to this previous sentence

However, verifying this condition
%%CF.4.30: what is "this condition"?
in large continuous state spaces
%%CF.4.30: the paper shows results in continuous state spaces. Not clear what you mean by "large"... I think the most convincing thing here would be to say that we compare to it and briefly foreshadow those results.
is non-trivial in most settings. To handle more general scenarios with potentially irreversible states, our setting allows the agent to request reset interventions. 
%%CF.4.30: I'm not sure if you need this last sentence... It's not super clear what the point is here.

%%CF.5.12: not sure, but you could add something like ", where the agent can detect irreversible states and ping a human expert for help."

%%CF.5.12: I think the above two sentences could be combined into one

% Constrained MDPs used in safe RL literature generally operates in the episodic settings assumes access to an oracle function indicating whether a state is safe or unsafe.

% SAILR \citep{wagener2021safe} requires a backup policy and the corresponding $Q$-value function corresponding to safety that can act safely with high probability when starting from the initial state distribution.

% Prior work has considered considered has an augmented MDP where the reward function penalizes \citep{wagener2021safe, thomas2021safe,sun2021safe} entry to unsafe states or whenever an intervention is invoked. Consequently, the policy learned in this unconstrained MDP (albeit with early termination whenever an unsafe state/intervention is encountered) will learn an optimal policy in the constrained MDP as well. However, we do not assume access to an oracle indicator function that indicates the safety of these states.

% SQRL, Learning to be safe conservatively, Recovery RL etc.. (Also more classical safe RL literature)

% \annie{Another line of safe RL research focuses on safety guarantees \emph{during} training. These methods can ensure the agent only takes actions that lead to next states that are safe~\citep{perkins2002lyapunov,berkenkamp2017safe,dalal2018safe,fisac2018general,thananjeyan2020safety} or construct a shielded policy that runs a backup policy if the agent proposes an unsafe action~\citep{alshiekh2018safe,turchetta2020safe,li2020robust,wagener2021safe}.}

% \annie{Constraint inference stuff}

% Closest to our framework is leave no trace (LNT) \citep{eysenbach2017leave} that learns a backward policy that resets the agent to the initial state distribution, and uses the estimated success of the backward policy to constrain the forward policy. However, LNT assumes access to an oracle function that indicates whether the backward policy was successful or not. LNT calls for an extrinsic intervention to reset the environment whenever the backward policy fails to reset the agent. This could be either because the agent is an irreversible state or because the backward policy was insufficiently trained.

% SAVED \citep{thananjeyan2020safety} is a model-based learning algorithm that leverages demonstrations to optimize sparse cost reward functions while being safe. SAVED constrains visitation to states such that the MPC controller can plan a sequence of actions to return to the "feasible region", where feasible region is defined as the set of states that are known to be able to reach the goal state (demos, previous online trajectories that reached the goal).

% Is there any literature that actively queries the safety of a state instead of assuming the oracle nature of ? There probably isn't because it is weird violate constraints that you might not even know (so there probably isn't literature on this). It might be nice to discuss this more in the context of irreversibility.

% Autonomous RL literature ... All prior work in this literature has confined itself to reversible/ergodic environments, not explicitly requiring the need to query or call a human. We extend the framework to non-ergodic environments and develop algorithms for it.

% - Episodic RL (choose 3 different \# of resets, e.g., 100, 1000, 10000, and the \# of resets used by our method)
% - Safe episodic RL (R min, critic, CPO) (choose 3 different \# of resets, e.g., 100, 1000, 10000, and the \# of resets used by our method)
% - MEDAL (use the same \# of resets as our method)
% - MEDAL + R min (oracle labels)
% - Leave No Trace (no labels)
% - Ours with self-supervised reversibility estimator (no labels)
% Ablation (mug env): episodic version of Ours with no early termination (use the same \# of resets as our method)
% Ablation (mug env): MEDAL + R min (fewer labels)


% To first analyze our algorithm and baselines in a simplified control task, we design an \emph{episodic} 2D continuous maze environment. Instead of walls, there are trenches throughout the maze (the positions of which are unknown to the agent a priori) which represent groups of connected irreversible states: the agent can fall into a trench, and once entered, it can roam freely within the trench but cannot leave it without an environment reset. 
% For evaluation in more complex tasks, we modify the Tabletop Organization and Peg Insertion environments from the EARL benchmark~\citep{sharma2021autonomous}. While the original tasks are designed for autonomous RL evaluation, we introduce irreversible states to each environment that reflect realistic examples of irreversibility, such as a robotic agent pushing an object out of its workspace. Following the evaluation protocol from the EARL benchmark, each of these tasks, including the maze environment, is to be solved from sparse rewards and a small number of demonstrations for the forward policy. 
% Finally, we design a \emph{continuing} task in the Half-Cheetah environment from OpenAI Gym~\citep{brockman2016openai}

% - Termination threshold: initial value-based, constants, adaptive (based on value of demo states?)
% - R min
% - Safety critic's epsilon
% - Pseudo-labels for unlabeled states: discriminator prediction, ratio of reversible to irreversible states in replay buffer, 0, 0.5, 1
% - Number of exploration steps
% - Number of demonstrations / availability of demonstrations
% - Shielding vs no shielding

% \subsection{Relaxing Assumptions}
% \textbf{Fully-reversible environment}.
